Impacting the dayside Martian ionosphere from above and below: Effects of the impact of CIRs and ICMEs close to aphelion (April 2021) and during dust storms (June-July 2022) seen with MAVEN ROSE

We use 62 electron density profiles collected by the Radio Occultation Science Experiment (ROSE), on MAVEN, when Mars was hit by CIRs and ICMEs close to aphelion (April 2021) and during two dust storms (June-July 2022) to examine the response of the Martian ionosphere to solar events and to solar events hitting during dust storms. We do so through three proxies - variation in total electron content between 80 and 300 km altitude, peak density, and peak altitude - of the aforementioned 62 ROSE electron density profiles, relative to a characterisation of the ionosphere through solar minimum leading to solar maximum, specific to local time sector and season, presented in Segale et al., (COMPANION). We observe an increased Total Electron Content (TEC) between 80 and 300 km altitude up to 2.5 x 10(15) m(-2) in April 2021 and up to 5 x 10(15) m(-2) in June-July 2022 compared to the baseline photochemically produced ionosphere. This increase in TEC corresponds mainly to increases in the solar energetic particles flux (detected by MAVEN SEP) and electron fluxes (detected by MAVEN SWEA). In addition to solar events, in June-July 2022, an A storm and a B storm were occurring and merging on the surface of Mars. We observe a raise in peak altitude in general lower than expected during dust storms, possibly due to high values of solar wind dynamic pressure (derived from MAVEN SWIA). From 31 ROSE profiles collected in this time period that showed both the M2 and M1 layer, we observe that, on average, M1 and M2 peak altitudes raise the same amount, suggesting that the thermosphere might loft as a unit during dust storms. During this time period, several proton aurora events of variable brightness were detected with MAVEN IUVS underlining the complex and multifaceted impact of dust activity and extreme solar activity on the Martian ionosphere.

==> main_bbl.tex <==
\begin{thebibliography}{51}
\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi
\providecommand{\url}[1]{\texttt{#1}}
\providecommand{\href}[2]{#2}
\providecommand{\path}[1]{#1}
\providecommand{\DOIprefix}{doi:}
\providecommand{\ArXivprefix}{arXiv:}
\providecommand{\URLprefix}{URL: }
\providecommand{\Pubmedprefix}{pmid:}
\providecommand{\doi}[1]{\href{http://dx.doi.org/#1}{\path{#1}}}
\providecommand{\Pubmed}[1]{\href{pmid:#1}{\path{#1}}}
\providecommand{\bibinfo}[2]{#2}
\ifx\xfnm\relax \def\xfnm[#1]{\unskip,\space#1}\fi
%Type = Book
\bibitem[{Barth et~al.(1992)Barth, I.~F.~Stewart, Bougher, M.~Hunten, Bauer and Nagy}]{Barth:1992aa}
\bibinfo{author}{Barth, C.}, \bibinfo{author}{I.~F.~Stewart, A.}, \bibinfo{author}{Bougher, S.W.}, \bibinfo{author}{M.~Hunten, D.}, \bibinfo{author}{Bauer, S.}, \bibinfo{author}{Nagy, A.}, \bibinfo{year}{1992}.
\newblock \bibinfo{title}{Aeronomy of the {C}urrent {M}artian {A}tmosphere}.
%Type = Inbook
\bibitem[{Bougher et~al.(2017)Bougher, Brain, Fox, Francisco, Simon-Wedlund and Withers}]{Bougher:2017}
\bibinfo{author}{Bougher, S.W.}, \bibinfo{author}{Brain, D.A.}, \bibinfo{author}{Fox, J.L.}, \bibinfo{author}{Francisco, G.G.}, \bibinfo{author}{Simon-Wedlund, C.}, \bibinfo{author}{Withers, P.G.}, \bibinfo{year}{2017}.
\newblock \bibinfo{title}{Upper Neutral Atmosphere and Ionosphere}. \bibinfo{publisher}{Cambridge University Press}.
\newblock Cambridge Planetary Science, pp. \bibinfo{pages}{433--463}.
\newblock \DOIprefix\doi{10.1017/9781139060172.014}.
%Type = Article
\bibitem[{Chaffin et~al.(2021)Chaffin, Kass, Aoki, Fedorova, Deighan, Connour, Heavens, Kleinb{\"o}hl, Jain, Chaufray, Mayyasi, Clarke, Stewart, Evans, Stevens, McClintock, Crismani, Holsclaw, Lefevre, Lo, Montmessin, Schneider, Jakosky, Villanueva, Liuzzi, Daerden, Thomas, Lopez-Moreno, Patel, Bellucci, Ristic, Erwin, Vandaele, Trokhimovskiy and Korablev}]{Chaffin:2021aa}
\bibinfo{author}{Chaffin, M.S.}, \bibinfo{author}{Kass, D.M.}, \bibinfo{author}{Aoki, S.}, \bibinfo{author}{Fedorova, A.A.}, \bibinfo{author}{Deighan, J.}, \bibinfo{author}{Connour, K.}, \bibinfo{author}{Heavens, N.G.}, \bibinfo{author}{Kleinb{\"o}hl, A.}, \bibinfo{author}{Jain, S.K.}, \bibinfo{author}{Chaufray, J.Y.}, \bibinfo{author}{Mayyasi, M.}, \bibinfo{author}{Clarke, J.T.}, \bibinfo{author}{Stewart, A.I.F.}, \bibinfo{author}{Evans, J.S.}, \bibinfo{author}{Stevens, M.H.}, \bibinfo{author}{McClintock, W.E.}, \bibinfo{author}{Crismani, M.M.J.}, \bibinfo{author}{Holsclaw, G.M.}, \bibinfo{author}{Lefevre, F.}, \bibinfo{author}{Lo, D.Y.}, \bibinfo{author}{Montmessin, F.}, \bibinfo{author}{Schneider, N.M.}, \bibinfo{author}{Jakosky, B.}, \bibinfo{author}{Villanueva, G.}, \bibinfo{author}{Liuzzi, G.}, \bibinfo{author}{Daerden, F.}, \bibinfo{author}{Thomas, I.R.}, \bibinfo{author}{Lopez-Moreno, J.J.}, \bibinfo{author}{Patel, M.R.}, \bibinfo{author}{Bellucci, G.}, \bibinfo{author}{Ristic, B.},
  \bibinfo{author}{Erwin, J.T.}, \bibinfo{author}{Vandaele, A.C.}, \bibinfo{author}{Trokhimovskiy, A.}, \bibinfo{author}{Korablev, O.I.}, \bibinfo{year}{2021}.
\newblock \bibinfo{title}{{Martian water loss to space enhanced by regional dust storms}}.
\newblock \bibinfo{journal}{Nature Astronomy} \bibinfo{volume}{5}, \bibinfo{pages}{1036--1042}.
\newblock \URLprefix \url{https://doi.org/10.1038/s41550-021-01425-w}, \DOIprefix\doi{10.1038/s41550-021-01425-w}.
%Type = Book
\bibitem[{Chamberlain and Hunten(1987)}]{Chamb:1987}
\bibinfo{author}{Chamberlain, J.}, \bibinfo{author}{Hunten, D.}, \bibinfo{year}{1987}.
\newblock \bibinfo{title}{Theory of {P}lanetary {A}tmospheres}.
\newblock \bibinfo{edition}{second ed.} ed., \bibinfo{publisher}{Academic Press, New York}.
%Type = Article
\bibitem[{Deighan et~al.(2018)Deighan, Jain, Chaffin, Fang, Halekas, Clarke, Schneider, Stewart, Chaufray, Evans, Stevens, Mayyasi, Stiepen, Crismani, McClintock, Holsclaw, Lo, Montmessin, Lef{\`e}vre and Jakosky}]{Deighan:2018aa}
\bibinfo{author}{Deighan, J.}, \bibinfo{author}{Jain, S.K.}, \bibinfo{author}{Chaffin, M.S.}, \bibinfo{author}{Fang, X.}, \bibinfo{author}{Halekas, J.S.}, \bibinfo{author}{Clarke, J.T.}, \bibinfo{author}{Schneider, N.M.}, \bibinfo{author}{Stewart, A.I.F.}, \bibinfo{author}{Chaufray, J.Y.}, \bibinfo{author}{Evans, J.S.}, \bibinfo{author}{Stevens, M.H.}, \bibinfo{author}{Mayyasi, M.}, \bibinfo{author}{Stiepen, A.}, \bibinfo{author}{Crismani, M.}, \bibinfo{author}{McClintock, W.E.}, \bibinfo{author}{Holsclaw, G.M.}, \bibinfo{author}{Lo, D.Y.}, \bibinfo{author}{Montmessin, F.}, \bibinfo{author}{Lef{\`e}vre, F.}, \bibinfo{author}{Jakosky, B.M.}, \bibinfo{year}{2018}.
\newblock \bibinfo{title}{{Discovery of a proton aurora at Mars}}.
\newblock \bibinfo{journal}{Nature Astronomy} \bibinfo{volume}{2}, \bibinfo{pages}{802--807}.
\newblock \URLprefix \url{https://doi.org/10.1038/s41550-018-0538-5}, \DOIprefix\doi{10.1038/s41550-018-0538-5}.
%Type = Article
\bibitem[{Dresing et~al.(2023)Dresing, Rodr{\'\i}guez-Garc{\'\i}a, Jebaraj, Warmuth, Wallace, Balmaceda, Podladchikova, Strauss, Kouloumvakos, Palmroos, Krupar, Gieseler, Xu, Mitchell, Cohen, de~Nolfo, Palmerio, Carcaboso, Kilpua, Trotta, Auster, Asvestari, da~Silva, Dr{\"o}ge, Getachew, G{\'o}mez-Herrero, Grande, Heyner, Holmstr{\"o}m, Huovelin, Kartavykh, Laurenza, Lee, Mason, Maksimovic, Mieth, Murakami, Oleynik, Pinto, Pulupa, Richter, Rodr{\'\i}guez-Pacheco, S{\'a}nchez-Cano, Schuller, Ueno, Vainio, Vecchio, Veronig and Wijsen}]{Dresing:2023aa}
\bibinfo{author}{Dresing, N.}, \bibinfo{author}{Rodr{\'\i}guez-Garc{\'\i}a, L.}, \bibinfo{author}{Jebaraj, I.C.}, \bibinfo{author}{Warmuth, A.}, \bibinfo{author}{Wallace, S.}, \bibinfo{author}{Balmaceda, L.}, \bibinfo{author}{Podladchikova, T.}, \bibinfo{author}{Strauss, R.D.}, \bibinfo{author}{Kouloumvakos, A.}, \bibinfo{author}{Palmroos, C.}, \bibinfo{author}{Krupar, V.}, \bibinfo{author}{Gieseler, J.}, \bibinfo{author}{Xu, Z.}, \bibinfo{author}{Mitchell, J.G.}, \bibinfo{author}{Cohen, C.M.S.}, \bibinfo{author}{de~Nolfo, G.A.}, \bibinfo{author}{Palmerio, E.}, \bibinfo{author}{Carcaboso, F.}, \bibinfo{author}{Kilpua, E.K.J.}, \bibinfo{author}{Trotta, D.}, \bibinfo{author}{Auster, U.}, \bibinfo{author}{Asvestari, E.}, \bibinfo{author}{da~Silva, D.}, \bibinfo{author}{Dr{\"o}ge, W.}, \bibinfo{author}{Getachew, T.}, \bibinfo{author}{G{\'o}mez-Herrero, R.}, \bibinfo{author}{Grande, M.}, \bibinfo{author}{Heyner, D.}, \bibinfo{author}{Holmstr{\"o}m, M.}, \bibinfo{author}{Huovelin, J.}, \bibinfo{author}{Kartavykh,
  Y.}, \bibinfo{author}{Laurenza, M.}, \bibinfo{author}{Lee, C.O.}, \bibinfo{author}{Mason, G.}, \bibinfo{author}{Maksimovic, M.}, \bibinfo{author}{Mieth, J.}, \bibinfo{author}{Murakami, G.}, \bibinfo{author}{Oleynik, P.}, \bibinfo{author}{Pinto, M.}, \bibinfo{author}{Pulupa, M.}, \bibinfo{author}{Richter, I.}, \bibinfo{author}{Rodr{\'\i}guez-Pacheco, J.}, \bibinfo{author}{S{\'a}nchez-Cano, B.}, \bibinfo{author}{Schuller, F.}, \bibinfo{author}{Ueno, H.}, \bibinfo{author}{Vainio, R.}, \bibinfo{author}{Vecchio, A.}, \bibinfo{author}{Veronig, A.M.}, \bibinfo{author}{Wijsen, N.}, \bibinfo{year}{2023}.
\newblock \bibinfo{title}{{The 17 April 2021 widespread solar energetic particle event}}.
\newblock \bibinfo{journal}{A\&A} \bibinfo{volume}{674}.
\newblock \URLprefix \url{https://doi.org/10.1051/0004-6361/202345938}.
%Type = Article
\bibitem[{Dubinin et~al.(2009)Dubinin, Fraenz, Woch, Duru, Gurnett, Modolo, Barabash and Lundin}]{Dubinin:2009aa}
\bibinfo{author}{Dubinin, E.}, \bibinfo{author}{Fraenz, M.}, \bibinfo{author}{Woch, J.}, \bibinfo{author}{Duru, F.}, \bibinfo{author}{Gurnett, D.}, \bibinfo{author}{Modolo, R.}, \bibinfo{author}{Barabash, S.}, \bibinfo{author}{Lundin, R.}, \bibinfo{year}{2009}.
\newblock \bibinfo{title}{Ionospheric storms on {M}ars: {I}mpact of the corotating interaction region}.
\newblock \bibinfo{journal}{Geophysical Research Letters} \bibinfo{volume}{36}.
\newblock \URLprefix \url{https://doi.org/10.1029/2008GL036559}, \DOIprefix\doi{https://doi.org/10.1029/2008GL036559}.
%Type = Article
\bibitem[{Edberg et~al.(2010)Edberg, Nilsson, Williams, Lester, Milan, Cowley, Fr{\"a}nz, Barabash and Futaana}]{Edberg:2010aa}
\bibinfo{author}{Edberg, N.J.T.}, \bibinfo{author}{Nilsson, H.}, \bibinfo{author}{Williams, A.O.}, \bibinfo{author}{Lester, M.}, \bibinfo{author}{Milan, S.E.}, \bibinfo{author}{Cowley, S.W.H.}, \bibinfo{author}{Fr{\"a}nz, M.}, \bibinfo{author}{Barabash, S.}, \bibinfo{author}{Futaana, Y.}, \bibinfo{year}{2010}.
\newblock \bibinfo{title}{Pumping out the atmosphere of {M}ars through solar wind pressure pulses}.
\newblock \bibinfo{journal}{Geophysical Research Letters} \bibinfo{volume}{37}.
\newblock \URLprefix \url{https://doi.org/10.1029/2009GL041814}, \DOIprefix\doi{https://doi.org/10.1029/2009GL041814}.
%Type = Article
\bibitem[{Ehresmann et~al.(2018)Ehresmann, Hassler, Zeitlin, Guo, Wimmer-Schweingruber, Matthi{\"a}, Lohf, Burmeister, Rafkin, Berger and Reitz}]{Ehresmann:2018aa}
\bibinfo{author}{Ehresmann, B.}, \bibinfo{author}{Hassler, D.M.}, \bibinfo{author}{Zeitlin, C.}, \bibinfo{author}{Guo, J.}, \bibinfo{author}{Wimmer-Schweingruber, R.F.}, \bibinfo{author}{Matthi{\"a}, D.}, \bibinfo{author}{Lohf, H.}, \bibinfo{author}{Burmeister, S.}, \bibinfo{author}{Rafkin, S.C.R.}, \bibinfo{author}{Berger, T.}, \bibinfo{author}{Reitz, G.}, \bibinfo{year}{2018}.
\newblock \bibinfo{title}{Energetic particle radiation environment observed by rad on the surface of mars during the september 2017 event}.
\newblock \bibinfo{journal}{Geophysical Research Letters} \bibinfo{volume}{45}, \bibinfo{pages}{5305--5311}.
\newblock \URLprefix \url{https://doi.org/10.1029/2018GL077801}, \DOIprefix\doi{https://doi.org/10.1029/2018GL077801}.
%Type = Article
\bibitem[{Eparvier et~al.(2015)Eparvier, Chamberlin, Woods and Thiemann}]{Eparvier:2015wc}
\bibinfo{author}{Eparvier, F.G.}, \bibinfo{author}{Chamberlin, P.C.}, \bibinfo{author}{Woods, T.N.}, \bibinfo{author}{Thiemann, E.M.B.}, \bibinfo{year}{2015}.
\newblock \bibinfo{title}{The solar extreme ultraviolet monitor for {M}{A}{V}{E}{N}}.
\newblock \bibinfo{journal}{Space Science Reviews} \bibinfo{volume}{195}, \bibinfo{pages}{293--301}.
\newblock \URLprefix \url{https://doi.org/10.1007/s11214-015-0195-2}, \DOIprefix\doi{10.1007/s11214-015-0195-2}.
%Type = Article
\bibitem[{{Fallows} et~al.(2015){Fallows}, {Withers} and {Matta}}]{fallows2015a}
\bibinfo{author}{{Fallows}, K.}, \bibinfo{author}{{Withers}, P.}, \bibinfo{author}{{Matta}, M.}, \bibinfo{year}{2015}.
\newblock \bibinfo{title}{{An observational study of the influence of solar zenith angle on properties of the M1 layer of the Mars ionosphere}}.
\newblock \bibinfo{journal}{J. Geophys. Res.} \bibinfo{volume}{120}, \bibinfo{pages}{1299--1310}.
\newblock \DOIprefix\doi{10.1002/2014JA020750}.
%Type = Article
\bibitem[{{Felici} et~al.(2020){Felici}, {Withers}, {Smith}, {Gonz{\'a}lez-Galindo}, {Oudrhiri} and {Kahan}}]{felici2020}
\bibinfo{author}{{Felici}, M.}, \bibinfo{author}{{Withers}, P.}, \bibinfo{author}{{Smith}, M.D.}, \bibinfo{author}{{Gonz{\'a}lez-Galindo}, F.}, \bibinfo{author}{{Oudrhiri}, K.}, \bibinfo{author}{{Kahan}, D.}, \bibinfo{year}{2020}.
\newblock \bibinfo{title}{{MAVEN ROSE Observations of the Response of the Martian Ionosphere to Dust Storms}}.
\newblock \bibinfo{journal}{Journal of Geophysical Research} \bibinfo{volume}{125}, \bibinfo{pages}{e27083}.
\newblock \DOIprefix\doi{10.1029/2019JA027083}.
%Type = Article
\bibitem[{Fox(2004)}]{Fox:2004aa}
\bibinfo{author}{Fox, J.L.}, \bibinfo{year}{2004}.
\newblock \bibinfo{title}{Response of the {M}artian thermosphere/ionosphere to enhanced fluxes of solar soft {X} rays}.
\newblock \bibinfo{journal}{Journal of Geophysical Research: Space Physics} \bibinfo{volume}{109}.
\newblock \URLprefix \url{https://doi.org/10.1029/2004JA010380}, \DOIprefix\doi{10.1029/2004JA010380}.
%Type = Misc
\bibitem[{Girazian et~al.(2019)Girazian, Luppen, Morgan, Chu, Montabone, Thiemann, Gurnett, Halekas, Kopf and Nemec}]{Girazian:2019}
\bibinfo{author}{Girazian, Z.}, \bibinfo{author}{Luppen, Z.}, \bibinfo{author}{Morgan, D.D.}, \bibinfo{author}{Chu, F.}, \bibinfo{author}{Montabone, L.}, \bibinfo{author}{Thiemann, E.M.B.}, \bibinfo{author}{Gurnett, D.A.}, \bibinfo{author}{Halekas, J.}, \bibinfo{author}{Kopf, A.J.}, \bibinfo{author}{Nemec, F.}, \bibinfo{year}{2019}.
\newblock \bibinfo{title}{Variations in the ionospheric peak altitude at mars in response to dust storms: 13 years of observations from the mars express radar sounder}.
\newblock \href{http://arxiv.org/abs/1906.07111}{{\tt arXiv:1906.07111}}.
%Type = Article
\bibitem[{Halekas et~al.(2015)Halekas, Lillis, Mitchell, Cravens, Mazelle, Connerney, Espley, Mahaffy, Benna, Jakosky, Luhmann, McFadden, Larson, Harada and Ruhunusiri}]{Halekas:2015aa}
\bibinfo{author}{Halekas, J.S.}, \bibinfo{author}{Lillis, R.J.}, \bibinfo{author}{Mitchell, D.L.}, \bibinfo{author}{Cravens, T.E.}, \bibinfo{author}{Mazelle, C.}, \bibinfo{author}{Connerney, J.E.P.}, \bibinfo{author}{Espley, J.R.}, \bibinfo{author}{Mahaffy, P.R.}, \bibinfo{author}{Benna, M.}, \bibinfo{author}{Jakosky, B.M.}, \bibinfo{author}{Luhmann, J.G.}, \bibinfo{author}{McFadden, J.P.}, \bibinfo{author}{Larson, D.E.}, \bibinfo{author}{Harada, Y.}, \bibinfo{author}{Ruhunusiri, S.}, \bibinfo{year}{2015}.
\newblock \bibinfo{title}{{MAVEN observations of solar wind hydrogen deposition in the atmosphere of Mars}}.
\newblock \bibinfo{journal}{Geophysical Research Letters} \bibinfo{volume}{42}, \bibinfo{pages}{8901--8909}.
\newblock \URLprefix \url{https://doi.org/10.1002/2015GL064693}, \DOIprefix\doi{https://doi.org/10.1002/2015GL064693}.
%Type = Article
\bibitem[{Halekas et~al.(2017)Halekas, Ruhunusiri, Harada, Collinson, Mitchell, Mazelle, McFadden, Connerney, Espley, Eparvier, Luhmann and Jakosky}]{Halekas:2017aa}
\bibinfo{author}{Halekas, J.S.}, \bibinfo{author}{Ruhunusiri, S.}, \bibinfo{author}{Harada, Y.}, \bibinfo{author}{Collinson, G.}, \bibinfo{author}{Mitchell, D.L.}, \bibinfo{author}{Mazelle, C.}, \bibinfo{author}{McFadden, J.P.}, \bibinfo{author}{Connerney, J.E.P.}, \bibinfo{author}{Espley, J.R.}, \bibinfo{author}{Eparvier, F.}, \bibinfo{author}{Luhmann, J.G.}, \bibinfo{author}{Jakosky, B.M.}, \bibinfo{year}{2017}.
\newblock \bibinfo{title}{{Structure, dynamics, and seasonal variability of the Mars-solar wind interaction: MAVEN Solar Wind Ion Analyzer in-flight performance and science results}}.
\newblock \bibinfo{journal}{Journal of Geophysical Research: Space Physics} \bibinfo{volume}{122}, \bibinfo{pages}{547--578}.
\newblock \URLprefix \url{https://doi.org/10.1002/2016JA023167}, \DOIprefix\doi{https://doi.org/10.1002/2016JA023167}.
%Type = Article
\bibitem[{{Halekas} et~al.(2015){Halekas}, {Taylor}, {Dalton}, {Johnson}, {Curtis}, {McFadden}, {Mitchell}, {Lin} and {Jakosky}}]{halekas2015}
\bibinfo{author}{{Halekas}, J.S.}, \bibinfo{author}{{Taylor}, E.R.}, \bibinfo{author}{{Dalton}, G.}, \bibinfo{author}{{Johnson}, G.}, \bibinfo{author}{{Curtis}, D.W.}, \bibinfo{author}{{McFadden}, J.P.}, \bibinfo{author}{{Mitchell}, D.L.}, \bibinfo{author}{{Lin}, R.P.}, \bibinfo{author}{{Jakosky}, B.M.}, \bibinfo{year}{2015}.
\newblock \bibinfo{title}{{The Solar Wind Ion Analyzer for MAVEN}}.
\newblock \bibinfo{journal}{Space Sci. Rev.} \bibinfo{volume}{195}, \bibinfo{pages}{125--151}.
\newblock \DOIprefix\doi{10.1007/s11214-013-0029-z}.
%Type = Article
\bibitem[{Harada et~al.(2023)Harada, Nakamura, S{\'a}nchez-Cano, Lester, Terada and Leblanc}]{Harada:2023aa}
\bibinfo{author}{Harada, Y.}, \bibinfo{author}{Nakamura, Y.}, \bibinfo{author}{S{\'a}nchez-Cano, B.}, \bibinfo{author}{Lester, M.}, \bibinfo{author}{Terada, N.}, \bibinfo{author}{Leblanc, F.}, \bibinfo{year}{2023}.
\newblock \bibinfo{title}{{Radio Absorption in the Nightside Ionosphere of Mars During Solar Energetic Particle Events}}.
\newblock \bibinfo{journal}{Space Weather} \bibinfo{volume}{21}, \bibinfo{pages}{e2023SW003755}.
\newblock \URLprefix \url{https://doi.org/10.1029/2023SW003755}, \DOIprefix\doi{https://doi.org/10.1029/2023SW003755}.
%Type = Article
\bibitem[{Hughes et~al.(2019)Hughes, Chaffin, Mierkiewicz, Deighan, Jain, Schneider, Mayyasi and Jakosky}]{Hughes:2019aa}
\bibinfo{author}{Hughes, A.}, \bibinfo{author}{Chaffin, M.}, \bibinfo{author}{Mierkiewicz, E.}, \bibinfo{author}{Deighan, J.}, \bibinfo{author}{Jain, S.}, \bibinfo{author}{Schneider, N.}, \bibinfo{author}{Mayyasi, M.}, \bibinfo{author}{Jakosky, B.}, \bibinfo{year}{2019}.
\newblock \bibinfo{title}{{Proton Aurora on Mars: A Dayside Phenomenon Pervasive in Southern Summer}}.
\newblock \bibinfo{journal}{Journal of Geophysical Research: Space Physics} \bibinfo{volume}{124}, \bibinfo{pages}{10533--10548}.
\newblock \URLprefix \url{https://doi.org/10.1029/2019JA027140}, \DOIprefix\doi{https://doi.org/10.1029/2019JA027140}.
%Type = Article
\bibitem[{Jakosky et~al.(2015a)Jakosky, Grebowsky, Luhmann, Connerney, Eparvier, Ergun, Halekas, Larson, Mahaffy, McFadden, Mitchell, Schneider, Zurek, Bougher, Brain, Ma, Mazelle, Andersson, Andrews, Baird, Baker, Bell, Benna, Chaffin, Chamberlin, Chaufray, Clarke, Collinson, Combi, Crary, Cravens, Crismani, Curry, Curtis, Deighan, Delory, Dewey, DiBraccio, Dong, Dong, Dunn, Elrod, England, Eriksson, Espley, Evans, Fang, Fillingim, Fortier, Fowler, Fox, Gr{\"o}ller, Guzewich, Hara, Harada, Holsclaw, Jain, Jolitz, Leblanc, Lee, Lee, Lefevre, Lillis, Livi, Lo, Mayyasi, McClintock, McEnulty, Modolo, Montmessin, Morooka, Nagy, Olsen, Peterson, Rahmati, Ruhunusiri, Russell, Sakai, Sauvaud, Seki, Steckiewicz, Stevens, Stewart, Stiepen, Stone, Tenishev, Thiemann, Tolson, Toublanc, Vogt, Weber, Withers, Woods and Yelle}]{Jakosky:2015CME}
\bibinfo{author}{Jakosky, B.M.}, \bibinfo{author}{Grebowsky, J.M.}, \bibinfo{author}{Luhmann, J.G.}, \bibinfo{author}{Connerney, J.}, \bibinfo{author}{Eparvier, F.}, \bibinfo{author}{Ergun, R.}, \bibinfo{author}{Halekas, J.}, \bibinfo{author}{Larson, D.}, \bibinfo{author}{Mahaffy, P.}, \bibinfo{author}{McFadden, J.}, \bibinfo{author}{Mitchell, D.L.}, \bibinfo{author}{Schneider, N.}, \bibinfo{author}{Zurek, R.}, \bibinfo{author}{Bougher, S.}, \bibinfo{author}{Brain, D.}, \bibinfo{author}{Ma, Y.J.}, \bibinfo{author}{Mazelle, C.}, \bibinfo{author}{Andersson, L.}, \bibinfo{author}{Andrews, D.}, \bibinfo{author}{Baird, D.}, \bibinfo{author}{Baker, D.}, \bibinfo{author}{Bell, J.M.}, \bibinfo{author}{Benna, M.}, \bibinfo{author}{Chaffin, M.}, \bibinfo{author}{Chamberlin, P.}, \bibinfo{author}{Chaufray, Y.Y.}, \bibinfo{author}{Clarke, J.}, \bibinfo{author}{Collinson, G.}, \bibinfo{author}{Combi, M.}, \bibinfo{author}{Crary, F.}, \bibinfo{author}{Cravens, T.}, \bibinfo{author}{Crismani, M.}, \bibinfo{author}{Curry,
  S.}, \bibinfo{author}{Curtis, D.}, \bibinfo{author}{Deighan, J.}, \bibinfo{author}{Delory, G.}, \bibinfo{author}{Dewey, R.}, \bibinfo{author}{DiBraccio, G.}, \bibinfo{author}{Dong, C.}, \bibinfo{author}{Dong, Y.}, \bibinfo{author}{Dunn, P.}, \bibinfo{author}{Elrod, M.}, \bibinfo{author}{England, S.}, \bibinfo{author}{Eriksson, A.}, \bibinfo{author}{Espley, J.}, \bibinfo{author}{Evans, S.}, \bibinfo{author}{Fang, X.}, \bibinfo{author}{Fillingim, M.}, \bibinfo{author}{Fortier, K.}, \bibinfo{author}{Fowler, C.M.}, \bibinfo{author}{Fox, J.}, \bibinfo{author}{Gr{\"o}ller, H.}, \bibinfo{author}{Guzewich, S.}, \bibinfo{author}{Hara, T.}, \bibinfo{author}{Harada, Y.}, \bibinfo{author}{Holsclaw, G.}, \bibinfo{author}{Jain, S.K.}, \bibinfo{author}{Jolitz, R.}, \bibinfo{author}{Leblanc, F.}, \bibinfo{author}{Lee, C.O.}, \bibinfo{author}{Lee, Y.}, \bibinfo{author}{Lefevre, F.}, \bibinfo{author}{Lillis, R.}, \bibinfo{author}{Livi, R.}, \bibinfo{author}{Lo, D.}, \bibinfo{author}{Mayyasi, M.}, \bibinfo{author}{McClintock,
  W.}, \bibinfo{author}{McEnulty, T.}, \bibinfo{author}{Modolo, R.}, \bibinfo{author}{Montmessin, F.}, \bibinfo{author}{Morooka, M.}, \bibinfo{author}{Nagy, A.}, \bibinfo{author}{Olsen, K.}, \bibinfo{author}{Peterson, W.}, \bibinfo{author}{Rahmati, A.}, \bibinfo{author}{Ruhunusiri, S.}, \bibinfo{author}{Russell, C.T.}, \bibinfo{author}{Sakai, S.}, \bibinfo{author}{Sauvaud, J.A.}, \bibinfo{author}{Seki, K.}, \bibinfo{author}{Steckiewicz, M.}, \bibinfo{author}{Stevens, M.}, \bibinfo{author}{Stewart, A.I.F.}, \bibinfo{author}{Stiepen, A.}, \bibinfo{author}{Stone, S.}, \bibinfo{author}{Tenishev, V.}, \bibinfo{author}{Thiemann, E.}, \bibinfo{author}{Tolson, R.}, \bibinfo{author}{Toublanc, D.}, \bibinfo{author}{Vogt, M.}, \bibinfo{author}{Weber, T.}, \bibinfo{author}{Withers, P.}, \bibinfo{author}{Woods, T.}, \bibinfo{author}{Yelle, R.}, \bibinfo{year}{2015}a.
\newblock \bibinfo{title}{{MAVEN observations of the response of Mars to an interplanetary coronal mass ejection}}.
\newblock \bibinfo{journal}{Science} \bibinfo{volume}{350}, \bibinfo{pages}{aad0210}.
\newblock \URLprefix \url{https://www.science.org/doi/abs/10.1126/science.aad0210}, \DOIprefix\doi{10.1126/science.aad0210}, \href{http://arxiv.org/abs/https://www.science.org/doi/pdf/10.1126/science.aad0210}{{\tt arXiv:https://www.science.org/doi/pdf/10.1126/science.aad0210}}.
%Type = Article
\bibitem[{Jakosky et~al.(2015b)Jakosky, Lin, Grebowsky, Luhmann, Mitchell, Beutelschies, Priser, Acuna, Andersson, Baird, Baker, Bartlett, Benna, Bougher, Brain, Carson, Cauffman, Chamberlin, Chaufray, Cheatom, Clarke, Connerney, Cravens, Curtis, Delory, Demcak, DeWolfe, Eparvier, Ergun, Eriksson, Espley, Fang, Folta, Fox, Gomez-Rosa, Habenicht, Halekas, Holsclaw, Houghton, Howard, Jarosz, Jedrich, Johnson, Kasprzak, Kelley, King, Lankton, Larson, Leblanc, Lefevre, Lillis, Mahaffy, Mazelle, McClintock, McFadden, Mitchell, Montmessin, Morrissey, Peterson, Possel, Sauvaud, Schneider, Sidney, Sparacino, Stewart, Tolson, Toublanc, Waters, Woods, Yelle and Zurek}]{Jakosky:2015}
\bibinfo{author}{Jakosky, B.M.}, \bibinfo{author}{Lin, R.P.}, \bibinfo{author}{Grebowsky, J.M.}, \bibinfo{author}{Luhmann, J.G.}, \bibinfo{author}{Mitchell, D.F.}, \bibinfo{author}{Beutelschies, G.}, \bibinfo{author}{Priser, T.}, \bibinfo{author}{Acuna, M.}, \bibinfo{author}{Andersson, L.}, \bibinfo{author}{Baird, D.}, \bibinfo{author}{Baker, D.}, \bibinfo{author}{Bartlett, R.}, \bibinfo{author}{Benna, M.}, \bibinfo{author}{Bougher, S.}, \bibinfo{author}{Brain, D.}, \bibinfo{author}{Carson, D.}, \bibinfo{author}{Cauffman, S.}, \bibinfo{author}{Chamberlin, P.}, \bibinfo{author}{Chaufray, J.Y.}, \bibinfo{author}{Cheatom, O.}, \bibinfo{author}{Clarke, J.}, \bibinfo{author}{Connerney, J.}, \bibinfo{author}{Cravens, T.}, \bibinfo{author}{Curtis, D.}, \bibinfo{author}{Delory, G.}, \bibinfo{author}{Demcak, S.}, \bibinfo{author}{DeWolfe, A.}, \bibinfo{author}{Eparvier, F.}, \bibinfo{author}{Ergun, R.}, \bibinfo{author}{Eriksson, A.}, \bibinfo{author}{Espley, J.}, \bibinfo{author}{Fang, X.}, \bibinfo{author}{Folta,
  D.}, \bibinfo{author}{Fox, J.}, \bibinfo{author}{Gomez-Rosa, C.}, \bibinfo{author}{Habenicht, S.}, \bibinfo{author}{Halekas, J.}, \bibinfo{author}{Holsclaw, G.}, \bibinfo{author}{Houghton, M.}, \bibinfo{author}{Howard, R.}, \bibinfo{author}{Jarosz, M.}, \bibinfo{author}{Jedrich, N.}, \bibinfo{author}{Johnson, M.}, \bibinfo{author}{Kasprzak, W.}, \bibinfo{author}{Kelley, M.}, \bibinfo{author}{King, T.}, \bibinfo{author}{Lankton, M.}, \bibinfo{author}{Larson, D.}, \bibinfo{author}{Leblanc, F.}, \bibinfo{author}{Lefevre, F.}, \bibinfo{author}{Lillis, R.}, \bibinfo{author}{Mahaffy, P.}, \bibinfo{author}{Mazelle, C.}, \bibinfo{author}{McClintock, W.}, \bibinfo{author}{McFadden, J.}, \bibinfo{author}{Mitchell, D.L.}, \bibinfo{author}{Montmessin, F.}, \bibinfo{author}{Morrissey, J.}, \bibinfo{author}{Peterson, W.}, \bibinfo{author}{Possel, W.}, \bibinfo{author}{Sauvaud, J.A.}, \bibinfo{author}{Schneider, N.}, \bibinfo{author}{Sidney, W.}, \bibinfo{author}{Sparacino, S.}, \bibinfo{author}{Stewart, A.I.F.},
  \bibinfo{author}{Tolson, R.}, \bibinfo{author}{Toublanc, D.}, \bibinfo{author}{Waters, C.}, \bibinfo{author}{Woods, T.}, \bibinfo{author}{Yelle, R.}, \bibinfo{author}{Zurek, R.}, \bibinfo{year}{2015}b.
\newblock \bibinfo{title}{The {M}ars {A}tmosphere and {V}olatile {E}volution ({M}{A}{V}{E}{N}) {M}ission}.
\newblock \bibinfo{journal}{Space Science Reviews} \bibinfo{volume}{195}, \bibinfo{pages}{3--48}.
\newblock \URLprefix \url{https://doi.org/10.1007/s11214-015-0139-x}, \DOIprefix\doi{10.1007/s11214-015-0139-x}.
%Type = Article
\bibitem[{Jones et~al.(2020)Jones, Scott, Barnard, Highfield, Lintott and Baeten}]{Jones:2020aa}
\bibinfo{author}{Jones, S.R.}, \bibinfo{author}{Scott, C.J.}, \bibinfo{author}{Barnard, L.A.}, \bibinfo{author}{Highfield, R.}, \bibinfo{author}{Lintott, C.J.}, \bibinfo{author}{Baeten, E.}, \bibinfo{year}{2020}.
\newblock \bibinfo{title}{{The Visual Complexity of Coronal Mass Ejections Follows the Solar Cycle}}.
\newblock \bibinfo{journal}{Space Weather} \bibinfo{volume}{18}, \bibinfo{pages}{e2020SW002556}.
\newblock \URLprefix \url{https://doi.org/10.1029/2020SW002556}, \DOIprefix\doi{https://doi.org/10.1029/2020SW002556}.
%Type = Inbook
\bibitem[{Kahre et~al.(2017)Kahre, Murphy, Newman, Wilson, Cantor, Lemmon and Wolff}]{Kahre:2017aa}
\bibinfo{author}{Kahre, M.A.}, \bibinfo{author}{Murphy, J.R.}, \bibinfo{author}{Newman, C.E.}, \bibinfo{author}{Wilson, R.J.}, \bibinfo{author}{Cantor, B.A.}, \bibinfo{author}{Lemmon, M.T.}, \bibinfo{author}{Wolff, M.J.}, \bibinfo{year}{2017}.
\newblock \bibinfo{title}{The {M}ars {D}ust {C}ycle}.
\newblock pp. \bibinfo{pages}{229--294}.
\newblock \URLprefix \url{https://ui.adsabs.harvard.edu/abs/2017acm..book..229K}, \DOIprefix\doi{10.1017/9781139060172.010}.
%Type = Article
\bibitem[{Kass et~al.(2016)Kass, Kleinb\"{o}hl, McCleese, Schofield and Smith}]{Kass:2016aa}
\bibinfo{author}{Kass, D.M.}, \bibinfo{author}{Kleinb\"{o}hl, A.}, \bibinfo{author}{McCleese, D.J.}, \bibinfo{author}{Schofield, J.T.}, \bibinfo{author}{Smith, M.D.}, \bibinfo{year}{2016}.
\newblock \bibinfo{title}{Interannual similarity in the martian atmosphere during the dust storm season}.
\newblock \bibinfo{journal}{Geophysical Research Letters} \bibinfo{volume}{43}, \bibinfo{pages}{6111--6118}.
\newblock \URLprefix \url{https://doi.org/10.1002/2016GL068978}, \DOIprefix\doi{10.1002/2016GL068978}.
%Type = Article
\bibitem[{{Larson} et~al.(2015){Larson}, {Lillis}, {Lee}, {Dunn}, {Hatch}, {Robinson}, {Glaser}, {Chen}, {Curtis}, {Tiu}, {Lin}, {Luhmann} and {Jakosky}}]{larson2015}
\bibinfo{author}{{Larson}, D.E.}, \bibinfo{author}{{Lillis}, R.J.}, \bibinfo{author}{{Lee}, C.O.}, \bibinfo{author}{{Dunn}, P.A.}, \bibinfo{author}{{Hatch}, K.}, \bibinfo{author}{{Robinson}, M.}, \bibinfo{author}{{Glaser}, D.}, \bibinfo{author}{{Chen}, J.}, \bibinfo{author}{{Curtis}, D.}, \bibinfo{author}{{Tiu}, C.}, \bibinfo{author}{{Lin}, R.P.}, \bibinfo{author}{{Luhmann}, J.G.}, \bibinfo{author}{{Jakosky}, B.M.}, \bibinfo{year}{2015}.
\newblock \bibinfo{title}{{The MAVEN Solar Energetic Particle Investigation}}.
\newblock \bibinfo{journal}{Space Sci. Rev.} \bibinfo{volume}{195}, \bibinfo{pages}{153--172}.
\newblock \DOIprefix\doi{10.1007/s11214-015-0218-z}.
%Type = Article
\bibitem[{Lee et~al.(2018)Lee, Jakosky, Luhmann, Brain, Mays, Hassler, Holmstr{\"o}m, Larson, Mitchell, Mazelle and Halekas}]{Lee:2018aa}
\bibinfo{author}{Lee, C.O.}, \bibinfo{author}{Jakosky, B.M.}, \bibinfo{author}{Luhmann, J.G.}, \bibinfo{author}{Brain, D.A.}, \bibinfo{author}{Mays, M.L.}, \bibinfo{author}{Hassler, D.M.}, \bibinfo{author}{Holmstr{\"o}m, M.}, \bibinfo{author}{Larson, D.E.}, \bibinfo{author}{Mitchell, D.L.}, \bibinfo{author}{Mazelle, C.}, \bibinfo{author}{Halekas, J.S.}, \bibinfo{year}{2018}.
\newblock \bibinfo{title}{{Observations and Impacts of the 10 September 2017 Solar Events at Mars: An Overview and Synthesis of the Initial Results}}.
\newblock \bibinfo{journal}{Geophysical Research Letters} \bibinfo{volume}{45}, \bibinfo{pages}{8871--8885}.
\newblock \URLprefix \url{https://doi.org/10.1029/2018GL079162}, \DOIprefix\doi{https://doi.org/10.1029/2018GL079162}.
%Type = Article
\bibitem[{Leovy(2001)}]{Leovy:2001aa}
\bibinfo{author}{Leovy, C.}, \bibinfo{year}{2001}.
\newblock \bibinfo{title}{Weather and climate on {M}ars}.
\newblock \bibinfo{journal}{Nature} \bibinfo{volume}{412}, \bibinfo{pages}{245--249}.
\newblock \URLprefix \url{https://ui.adsabs.harvard.edu/abs/2001Natur.412..245L}.
%Type = Article
\bibitem[{Lester et~al.(2022)Lester, Sanchez-Cano, Potts, Lillis, Cartacci, Bernardini, Orosei, Perry, Putzig, Campbell, Blelly, Milan, Opgenoorth, Witasse, Redrojo and Russell}]{Lester:2022aa}
\bibinfo{author}{Lester, M.}, \bibinfo{author}{Sanchez-Cano, B.}, \bibinfo{author}{Potts, D.}, \bibinfo{author}{Lillis, R.}, \bibinfo{author}{Cartacci, M.}, \bibinfo{author}{Bernardini, F.}, \bibinfo{author}{Orosei, R.}, \bibinfo{author}{Perry, M.}, \bibinfo{author}{Putzig, N.}, \bibinfo{author}{Campbell, B.}, \bibinfo{author}{Blelly, P.L.}, \bibinfo{author}{Milan, S.}, \bibinfo{author}{Opgenoorth, H.}, \bibinfo{author}{Witasse, O.}, \bibinfo{author}{Redrojo, E.M.M.}, \bibinfo{author}{Russell, A.}, \bibinfo{year}{2022}.
\newblock \bibinfo{title}{{The Impact of Energetic Particles on the Martian Ionosphere During a Full Solar Cycle of Radar Observations: Radar Blackouts}}.
\newblock \bibinfo{journal}{Journal of Geophysical Research: Space Physics} \bibinfo{volume}{127}, \bibinfo{pages}{e2021JA029535}.
\newblock \URLprefix \url{https://doi.org/10.1029/2021JA029535}, \DOIprefix\doi{https://doi.org/10.1029/2021JA029535}.
%Type = Article
\bibitem[{McClintock et~al.(2015)McClintock, Schneider, Holsclaw, Clarke, Hoskins, Stewart, Montmessin, Yelle and Deighan}]{McClintock:2015aa}
\bibinfo{author}{McClintock, W.E.}, \bibinfo{author}{Schneider, N.M.}, \bibinfo{author}{Holsclaw, G.M.}, \bibinfo{author}{Clarke, J.T.}, \bibinfo{author}{Hoskins, A.C.}, \bibinfo{author}{Stewart, I.}, \bibinfo{author}{Montmessin, F.}, \bibinfo{author}{Yelle, R.V.}, \bibinfo{author}{Deighan, J.}, \bibinfo{year}{2015}.
\newblock \bibinfo{title}{{The Imaging Ultraviolet Spectrograph (IUVS) for the MAVEN Mission}}.
\newblock \bibinfo{journal}{Space Science Reviews} \bibinfo{volume}{195}, \bibinfo{pages}{75--124}.
\newblock \URLprefix \url{https://doi.org/10.1007/s11214-014-0098-7}, \DOIprefix\doi{10.1007/s11214-014-0098-7}.
%Type = Article
\bibitem[{{Mitchell} et~al.(2016){Mitchell}, {Mazelle}, {Sauvaud}, {Thocaven}, {Rouzaud}, {Fedorov}, {Rouger}, {Toublanc}, {Taylor}, {Gordon}, {Robinson}, {Heavner}, {Turin}, {Diaz-Aguado}, {Curtis}, {Lin} and {Jakosky}}]{mitchell2016}
\bibinfo{author}{{Mitchell}, D.L.}, \bibinfo{author}{{Mazelle}, C.}, \bibinfo{author}{{Sauvaud}, J.A.}, \bibinfo{author}{{Thocaven}, J.J.}, \bibinfo{author}{{Rouzaud}, J.}, \bibinfo{author}{{Fedorov}, A.}, \bibinfo{author}{{Rouger}, P.}, \bibinfo{author}{{Toublanc}, D.}, \bibinfo{author}{{Taylor}, E.}, \bibinfo{author}{{Gordon}, D.}, \bibinfo{author}{{Robinson}, M.}, \bibinfo{author}{{Heavner}, S.}, \bibinfo{author}{{Turin}, P.}, \bibinfo{author}{{Diaz-Aguado}, M.}, \bibinfo{author}{{Curtis}, D.W.}, \bibinfo{author}{{Lin}, R.P.}, \bibinfo{author}{{Jakosky}, B.M.}, \bibinfo{year}{2016}.
\newblock \bibinfo{title}{{The MAVEN Solar Wind Electron Analyzer}}.
\newblock \bibinfo{journal}{Space Sci. Rev.} \bibinfo{volume}{200}, \bibinfo{pages}{495--528}.
\newblock \DOIprefix\doi{10.1007/s11214-015-0232-1}.
%Type = Article
\bibitem[{Montabone et~al.(2015)Montabone, Forget, Millour, Wilson, Lewis, Cantor, Kass, Kleinb{\"o}hl, Lemmon, Smith and Wolff}]{Montabone:2015aa}
\bibinfo{author}{Montabone, L.}, \bibinfo{author}{Forget, F.}, \bibinfo{author}{Millour, E.}, \bibinfo{author}{Wilson, R.J.}, \bibinfo{author}{Lewis, S.R.}, \bibinfo{author}{Cantor, B.}, \bibinfo{author}{Kass, D.}, \bibinfo{author}{Kleinb{\"o}hl, A.}, \bibinfo{author}{Lemmon, M.T.}, \bibinfo{author}{Smith, M.D.}, \bibinfo{author}{Wolff, M.J.}, \bibinfo{year}{2015}.
\newblock \bibinfo{title}{Eight-year climatology of dust optical depth on mars}.
\newblock \bibinfo{journal}{Icarus} \bibinfo{volume}{251}, \bibinfo{pages}{65--95}.
\newblock \URLprefix \url{http://www.sciencedirect.com/science/article/pii/S0019103515000044}, \DOIprefix\doi{https://doi.org/10.1016/j.icarus.2014.12.034}.
%Type = Article
\bibitem[{Montabone et~al.(2020)Montabone, Spiga, Kass, Kleinb{\"o}hl, Forget and Millour}]{Montabone:2020aa}
\bibinfo{author}{Montabone, L.}, \bibinfo{author}{Spiga, A.}, \bibinfo{author}{Kass, D.M.}, \bibinfo{author}{Kleinb{\"o}hl, A.}, \bibinfo{author}{Forget, F.}, \bibinfo{author}{Millour, E.}, \bibinfo{year}{2020}.
\newblock \bibinfo{title}{Martian year 34 column dust climatology from mars climate sounder observations: Reconstructed maps and model simulations}.
\newblock \bibinfo{journal}{Journal of Geophysical Research: Planets} \bibinfo{volume}{n/a}, \bibinfo{pages}{e2019JE006111}.
\newblock \URLprefix \url{https://doi.org/10.1029/2019JE006111}, \DOIprefix\doi{10.1029/2019JE006111}.
%Type = Article
\bibitem[{Morgan et~al.(2014)Morgan, Di{\'e}val, Gurnett, Duru, Dubinin, Fr{\"a}nz, Andrews, Opgenoorth, Ulu{\c s}en, Mitrofanov and Plaut}]{Morgan:2014aa}
\bibinfo{author}{Morgan, D.D.}, \bibinfo{author}{Di{\'e}val, C.}, \bibinfo{author}{Gurnett, D.A.}, \bibinfo{author}{Duru, F.}, \bibinfo{author}{Dubinin, E.M.}, \bibinfo{author}{Fr{\"a}nz, M.}, \bibinfo{author}{Andrews, D.J.}, \bibinfo{author}{Opgenoorth, H.J.}, \bibinfo{author}{Ulu{\c s}en, D.}, \bibinfo{author}{Mitrofanov, I.}, \bibinfo{author}{Plaut, J.J.}, \bibinfo{year}{2014}.
\newblock \bibinfo{title}{{Effects of a strong ICME on the Martian ionosphere as detected by Mars Express and Mars Odyssey}}.
\newblock \bibinfo{journal}{Journal of Geophysical Research: Space Physics} \bibinfo{volume}{119}, \bibinfo{pages}{5891--5908}.
\newblock \URLprefix \url{https://doi.org/10.1002/2013JA019522}, \DOIprefix\doi{https://doi.org/10.1002/2013JA019522}.
%Type = Article
\bibitem[{Nakamura et~al.(2022)Nakamura, Terada, Leblanc, Rahmati, Nakagawa, Sakai, Hiruba, Kataoka and Murase}]{Nakamura:2022aa}
\bibinfo{author}{Nakamura, Y.}, \bibinfo{author}{Terada, N.}, \bibinfo{author}{Leblanc, F.}, \bibinfo{author}{Rahmati, A.}, \bibinfo{author}{Nakagawa, H.}, \bibinfo{author}{Sakai, S.}, \bibinfo{author}{Hiruba, S.}, \bibinfo{author}{Kataoka, R.}, \bibinfo{author}{Murase, K.}, \bibinfo{year}{2022}.
\newblock \bibinfo{title}{{Modeling of Diffuse Auroral Emission at Mars: Contribution of MeV Protons}}.
\newblock \bibinfo{journal}{Journal of Geophysical Research: Space Physics} \bibinfo{volume}{127}, \bibinfo{pages}{e2021JA029914}.
\newblock \URLprefix \url{https://doi.org/10.1029/2021JA029914}, \DOIprefix\doi{https://doi.org/10.1029/2021JA029914}.
%Type = Article
\bibitem[{Odstrcil(2003)}]{Odstrcil:2003aa}
\bibinfo{author}{Odstrcil, D.}, \bibinfo{year}{2003}.
\newblock \bibinfo{title}{{Modeling 3-D solar wind structure}}.
\newblock \bibinfo{journal}{Advances in Space Research} \bibinfo{volume}{32}, \bibinfo{pages}{497--506}.
\newblock \URLprefix \url{https://www.sciencedirect.com/science/article/pii/S0273117703003326}, \DOIprefix\doi{https://doi.org/10.1016/S0273-1177(03)00332-6}.
%Type = Article
\bibitem[{Opgenoorth et~al.(2013)Opgenoorth, Andrews, Fr{\"a}nz, Lester, Edberg, Morgan, Duru, Witasse and Williams}]{Opgenoorth:2013aa}
\bibinfo{author}{Opgenoorth, H.J.}, \bibinfo{author}{Andrews, D.J.}, \bibinfo{author}{Fr{\"a}nz, M.}, \bibinfo{author}{Lester, M.}, \bibinfo{author}{Edberg, N.J.T.}, \bibinfo{author}{Morgan, D.}, \bibinfo{author}{Duru, F.}, \bibinfo{author}{Witasse, O.}, \bibinfo{author}{Williams, A.O.}, \bibinfo{year}{2013}.
\newblock \bibinfo{title}{{Mars ionospheric response to solar wind variability}}.
\newblock \bibinfo{journal}{Journal of Geophysical Research: Space Physics} \bibinfo{volume}{118}, \bibinfo{pages}{6558--6587}.
\newblock \URLprefix \url{https://doi.org/10.1002/jgra.50537}, \DOIprefix\doi{https://doi.org/10.1002/jgra.50537}.
%Type = Article
\bibitem[{Owens(2018)}]{Owens:2018aa}
\bibinfo{author}{Owens, M.J.}, \bibinfo{year}{2018}.
\newblock \bibinfo{title}{{Solar Wind and Heavy Ion Properties of Interplanetary Coronal Mass Ejections}}.
\newblock \bibinfo{journal}{Solar Physics} \bibinfo{volume}{293}, \bibinfo{pages}{122}.
\newblock \URLprefix \url{https://doi.org/10.1007/s11207-018-1343-0}, \DOIprefix\doi{10.1007/s11207-018-1343-0}.
%Type = Article
\bibitem[{Palmerio et~al.(2021)Palmerio, Kilpua, Witasse, Barnes, S{\'a}nchez-Cano, Weiss, Nieves-Chinchilla, M{\"o}stl, Jian, Mierla, Zhukov, Guo, Rodriguez, Lowrance, Isavnin, Turc, Futaana and Holmstr{\"o}m}]{Palmerio:2021aa}
\bibinfo{author}{Palmerio, E.}, \bibinfo{author}{Kilpua, E.K.J.}, \bibinfo{author}{Witasse, O.}, \bibinfo{author}{Barnes, D.}, \bibinfo{author}{S{\'a}nchez-Cano, B.}, \bibinfo{author}{Weiss, A.J.}, \bibinfo{author}{Nieves-Chinchilla, T.}, \bibinfo{author}{M{\"o}stl, C.}, \bibinfo{author}{Jian, L.K.}, \bibinfo{author}{Mierla, M.}, \bibinfo{author}{Zhukov, A.N.}, \bibinfo{author}{Guo, J.}, \bibinfo{author}{Rodriguez, L.}, \bibinfo{author}{Lowrance, P.J.}, \bibinfo{author}{Isavnin, A.}, \bibinfo{author}{Turc, L.}, \bibinfo{author}{Futaana, Y.}, \bibinfo{author}{Holmstr{\"o}m, M.}, \bibinfo{year}{2021}.
\newblock \bibinfo{title}{{CME Magnetic Structure and IMF Preconditioning Affecting SEP Transport}}.
\newblock \bibinfo{journal}{Space Weather} \bibinfo{volume}{19}, \bibinfo{pages}{e2020SW002654}.
\newblock \URLprefix \url{https://doi.org/10.1029/2020SW002654}, \DOIprefix\doi{https://doi.org/10.1029/2020SW002654}.
%Type = Article
\bibitem[{Peter et~al.(2021)Peter, P{\"a}tzold, Molina-Cuberos, Gonz{\'a}lez-Galindo, Witasse, Tellmann, H{\"a}usler and Bird}]{Peter:2021aa}
\bibinfo{author}{Peter, K.}, \bibinfo{author}{P{\"a}tzold, M.}, \bibinfo{author}{Molina-Cuberos, G.J.}, \bibinfo{author}{Gonz{\'a}lez-Galindo, F.}, \bibinfo{author}{Witasse, O.}, \bibinfo{author}{Tellmann, S.}, \bibinfo{author}{H{\"a}usler, B.}, \bibinfo{author}{Bird, M.K.}, \bibinfo{year}{2021}.
\newblock \bibinfo{title}{{The lower dayside ionosphere of Mars from 14 years of MaRS radio science observations}}.
\newblock \bibinfo{journal}{Icarus} \bibinfo{volume}{359}, \bibinfo{pages}{114213}.
\newblock \URLprefix \url{https://www.sciencedirect.com/science/article/pii/S0019103520305455}, \DOIprefix\doi{https://doi.org/10.1016/j.icarus.2020.114213}.
%Type = Article
\bibitem[{Ram et~al.(2023)Ram, Rout, Rathi, Mondal, Sarkhel and Halekas}]{Ram:2023aa}
\bibinfo{author}{Ram, L.}, \bibinfo{author}{Rout, D.}, \bibinfo{author}{Rathi, R.}, \bibinfo{author}{Mondal, S.}, \bibinfo{author}{Sarkhel, S.}, \bibinfo{author}{Halekas, J.}, \bibinfo{year}{2023}.
\newblock \bibinfo{title}{{A Comparison of the Impacts of CMEs and CIRs on the Martian Dayside and Nightside Ionospheric Species}}.
\newblock \bibinfo{journal}{Journal of Geophysical Research: Planets} \bibinfo{volume}{128}, \bibinfo{pages}{e2022JE007649}.
\newblock \URLprefix \url{https://doi.org/10.1029/2022JE007649}, \DOIprefix\doi{https://doi.org/10.1029/2022JE007649}.
%Type = Article
\bibitem[{Richardson(2018)}]{Richardson:2018aa}
\bibinfo{author}{Richardson, I.G.}, \bibinfo{year}{2018}.
\newblock \bibinfo{title}{Solar wind stream interaction regions throughout the heliosphere}.
\newblock \bibinfo{journal}{Living Reviews in Solar Physics} \bibinfo{volume}{15}, \bibinfo{pages}{1}.
\newblock \URLprefix \url{https://doi.org/10.1007/s41116-017-0011-z}, \DOIprefix\doi{10.1007/s41116-017-0011-z}.
%Type = Article
\bibitem[{S{\'a}nchez-Cano et~al.(2019)S{\'a}nchez-Cano, Blelly, Lester, Witasse, Cartacci, Orosei, Opgenoorth, Lillis, Leblanc, Milan, Conroy, Floury, Plane, Cicchetti, Noschese and Kopf}]{SanchezCano:2019aa}
\bibinfo{author}{S{\'a}nchez-Cano, B.}, \bibinfo{author}{Blelly, P.L.}, \bibinfo{author}{Lester, M.}, \bibinfo{author}{Witasse, O.}, \bibinfo{author}{Cartacci, M.}, \bibinfo{author}{Orosei, R.}, \bibinfo{author}{Opgenoorth, H.}, \bibinfo{author}{Lillis, R.}, \bibinfo{author}{Leblanc, F.}, \bibinfo{author}{Milan, S.E.}, \bibinfo{author}{Conroy, P.}, \bibinfo{author}{Floury, N.}, \bibinfo{author}{Plane, J.M.C.}, \bibinfo{author}{Cicchetti, A.}, \bibinfo{author}{Noschese, R.}, \bibinfo{author}{Kopf, A.J.}, \bibinfo{year}{2019}.
\newblock \bibinfo{title}{{Origin of the Extended Mars Radar Blackout of September 2017}}.
\newblock \bibinfo{journal}{Journal of Geophysical Research: Space Physics} \bibinfo{volume}{124}, \bibinfo{pages}{4556--4568}.
\newblock \URLprefix \url{https://doi.org/10.1029/2018JA026403}, \DOIprefix\doi{https://doi.org/10.1029/2018JA026403}.
%Type = Article
\bibitem[{S{\'a}nchez-Cano et~al.(2017)S{\'a}nchez-Cano, Hall, Lester, Mays, Witasse, Ambrosi, Andrews, Cartacci, Cicchetti, Holmstr{\"o}m, Imber, Kajdi{\v c}, Milan, Noschese, Odstrcil, Opgenoorth, Plaut, Ramstad and Reyes-Ayala}]{Sanchez-Cano:2017aa}
\bibinfo{author}{S{\'a}nchez-Cano, B.}, \bibinfo{author}{Hall, B.E.S.}, \bibinfo{author}{Lester, M.}, \bibinfo{author}{Mays, M.L.}, \bibinfo{author}{Witasse, O.}, \bibinfo{author}{Ambrosi, R.}, \bibinfo{author}{Andrews, D.}, \bibinfo{author}{Cartacci, M.}, \bibinfo{author}{Cicchetti, A.}, \bibinfo{author}{Holmstr{\"o}m, M.}, \bibinfo{author}{Imber, S.}, \bibinfo{author}{Kajdi{\v c}, P.}, \bibinfo{author}{Milan, S.E.}, \bibinfo{author}{Noschese, R.}, \bibinfo{author}{Odstrcil, D.}, \bibinfo{author}{Opgenoorth, H.}, \bibinfo{author}{Plaut, J.}, \bibinfo{author}{Ramstad, R.}, \bibinfo{author}{Reyes-Ayala, K.I.}, \bibinfo{year}{2017}.
\newblock \bibinfo{title}{{Mars plasma system response to solar wind disturbances during solar minimum}}.
\newblock \bibinfo{journal}{Journal of Geophysical Research: Space Physics} \bibinfo{volume}{122}, \bibinfo{pages}{6611--6634}.
\newblock \URLprefix \url{https://doi.org/10.1002/2016JA023587}, \DOIprefix\doi{https://doi.org/10.1002/2016JA023587}.
%Type = Article
\bibitem[{Ulusen et~al.(2012)Ulusen, Brain, Luhmann and Mitchell}]{Ulusen:2012aa}
\bibinfo{author}{Ulusen, D.}, \bibinfo{author}{Brain, D.A.}, \bibinfo{author}{Luhmann, J.G.}, \bibinfo{author}{Mitchell, D.L.}, \bibinfo{year}{2012}.
\newblock \bibinfo{title}{{Investigation of Mars' ionospheric response to solar energetic particle events}}.
\newblock \bibinfo{journal}{Journal of Geophysical Research: Space Physics} \bibinfo{volume}{117}.
\newblock \URLprefix \url{https://doi.org/10.1029/2012JA017671}, \DOIprefix\doi{https://doi.org/10.1029/2012JA017671}.
%Type = Article
\bibitem[{Withers(2009)}]{Withers:2009aa}
\bibinfo{author}{Withers, P.}, \bibinfo{year}{2009}.
\newblock \bibinfo{title}{A review of observed variability in the dayside ionosphere of {M}ars}.
\newblock \bibinfo{journal}{Advances in Space Research} \bibinfo{volume}{44}, \bibinfo{pages}{277--307}.
\newblock \URLprefix \url{http://www.sciencedirect.com/science/article/pii/S0273117709002944}, \DOIprefix\doi{https://doi.org/10.1016/j.asr.2009.04.027}.
%Type = Article
\bibitem[{Withers et~al.(2023)Withers, Felici, Hensley, Mendillo, Barbinis, Kahan, Oudrhiri and Girazian}]{Withers:2023aa}
\bibinfo{author}{Withers, P.}, \bibinfo{author}{Felici, M.}, \bibinfo{author}{Hensley, K.}, \bibinfo{author}{Mendillo, M.}, \bibinfo{author}{Barbinis, E.}, \bibinfo{author}{Kahan, D.}, \bibinfo{author}{Oudrhiri, K.}, \bibinfo{author}{Girazian, Z.}, \bibinfo{year}{2023}.
\newblock \bibinfo{title}{{The ionosphere of Mars from solar minimum to solar maximum: Dayside electron densities from MAVEN and Mars Global Surveyor radio occultations}}.
\newblock \bibinfo{journal}{Icarus} \bibinfo{volume}{393}, \bibinfo{pages}{114508}.
\newblock \URLprefix \url{https://www.sciencedirect.com/science/article/pii/S0019103521001834}, \DOIprefix\doi{https://doi.org/10.1016/j.icarus.2021.114508}.
%Type = Article
\bibitem[{Withers et~al.(2018)Withers, Felici, Mendillo, Moore, Narvaez, Vogt and Jakosky}]{Withers:2018aa}
\bibinfo{author}{Withers, P.}, \bibinfo{author}{Felici, M.}, \bibinfo{author}{Mendillo, M.}, \bibinfo{author}{Moore, L.}, \bibinfo{author}{Narvaez, C.}, \bibinfo{author}{Vogt, M.F.}, \bibinfo{author}{Jakosky, B.M.}, \bibinfo{year}{2018}.
\newblock \bibinfo{title}{First {I}onospheric {R}esults {F}rom the {M}{A}{V}{E}{N} {R}adio {O}ccultation {S}cience {E}xperiment ({R}{O}{S}{E})}.
\newblock \bibinfo{journal}{Journal of Geophysical Research: Space Physics} \bibinfo{volume}{123}, \bibinfo{pages}{4171--4180}.
\newblock \URLprefix \url{https://doi.org/10.1029/2018JA025182}, \DOIprefix\doi{doi:10.1029/2018JA025182}.
%Type = Article
\bibitem[{Withers et~al.(2020)Withers, Felici, Mendillo, Moore, Narvaez, Vogt, Oudrhiri, Kahan and Jakosky}]{Withers:2020um}
\bibinfo{author}{Withers, P.}, \bibinfo{author}{Felici, M.}, \bibinfo{author}{Mendillo, M.}, \bibinfo{author}{Moore, L.}, \bibinfo{author}{Narvaez, C.}, \bibinfo{author}{Vogt, M.F.}, \bibinfo{author}{Oudrhiri, K.}, \bibinfo{author}{Kahan, D.}, \bibinfo{author}{Jakosky, B.M.}, \bibinfo{year}{2020}.
\newblock \bibinfo{title}{The maven radio occultation science experiment (rose)}.
\newblock \bibinfo{journal}{Space Science Reviews} \bibinfo{volume}{216}, \bibinfo{pages}{61}.
\newblock \URLprefix \url{https://doi.org/10.1007/s11214-020-00687-6}, \DOIprefix\doi{10.1007/s11214-020-00687-6}.
%Type = Article
\bibitem[{{Withers} and {Pratt}(2013)}]{withers2013}
\bibinfo{author}{{Withers}, P.}, \bibinfo{author}{{Pratt}, R.}, \bibinfo{year}{2013}.
\newblock \bibinfo{title}{{An observational study of the response of the upper atmosphere of Mars to lower atmospheric dust storms}}.
\newblock \bibinfo{journal}{Icarus} \bibinfo{volume}{225}, \bibinfo{pages}{378--389}.
\newblock \DOIprefix\doi{10.1016/j.icarus.2013.02.032}.
%Type = Article
\bibitem[{Zeitlin et~al.(2018)Zeitlin, Hassler, Guo, Ehresmann, Wimmer-Schweingruber, Rafkin, Freiherr~von Forstner, Lohf, Berger, Matthiae and Reitz}]{Zeitlin:2018aa}
\bibinfo{author}{Zeitlin, C.}, \bibinfo{author}{Hassler, D.M.}, \bibinfo{author}{Guo, J.}, \bibinfo{author}{Ehresmann, B.}, \bibinfo{author}{Wimmer-Schweingruber, R.F.}, \bibinfo{author}{Rafkin, S.C.R.}, \bibinfo{author}{Freiherr~von Forstner, J.L.}, \bibinfo{author}{Lohf, H.}, \bibinfo{author}{Berger, T.}, \bibinfo{author}{Matthiae, D.}, \bibinfo{author}{Reitz, G.}, \bibinfo{year}{2018}.
\newblock \bibinfo{title}{{Analysis of the Radiation Hazard Observed by RAD on the Surface of Mars During the September 2017 Solar Particle Event}}.
\newblock \bibinfo{journal}{Geophysical Research Letters} \bibinfo{volume}{45}, \bibinfo{pages}{5845--5851}.
\newblock \URLprefix \url{https://doi.org/10.1029/2018GL077760}, \DOIprefix\doi{https://doi.org/10.1029/2018GL077760}.
%Type = Article
\bibitem[{Zurbuchen and Richardson(2006)}]{Zurbuchen:2006aa}
\bibinfo{author}{Zurbuchen, T.H.}, \bibinfo{author}{Richardson, I.G.}, \bibinfo{year}{2006}.
\newblock \bibinfo{title}{{In-Situ Solar Wind and Magnetic Field Signatures of Interplanetary Coronal Mass Ejections}}.
\newblock \bibinfo{journal}{Space Science Reviews} \bibinfo{volume}{123}, \bibinfo{pages}{31--43}.
\newblock \URLprefix \url{https://doi.org/10.1007/s11214-006-9010-4}, \DOIprefix\doi{10.1007/s11214-006-9010-4}.

\end{thebibliography}

